Dual Prompting Image Restoration with Diffusion Transformers

Recent state-of-the-art image restoration methods mostly adopt latent diffusion models with U-Net backbones, yet still facing challenges in achieving high-quality restoration due to their limited capabilities. Diffusion transformers (DiTs), like SD3, are emerging as a promising alternative because of their better quality with scalability. In this paper, we introduce DPIR (Dual Prompting Image Restoration), a novel image restoration method that effectivly extracts conditional information of low-quality images from multiple perspectives. Specifically, DPIR consits of two branches: a low-quality image conditioning branch and a dual prompting control branch. The first branch utilizes a lightweight module to incorporate image priors into the DiT with high efficiency. More importantly, we believe that in image restoration, textual description alone cannot fully capture its rich visual characteristics. Therefore, a dual prompting module is designed to provide DiT with additional visual cues, capturing both global context and local appearance. The extracted global-local visual prompts as extra conditional control, alongside textual prompts to form dual prompts, greatly enhance the quality of the restoration. Extensive experimental results demonstrate that DPIR delivers superior image restoration performance.

==> tables/Kbjy_Q1.tex <==

%\begin{table}[htbp]
%\tiny
%\setlength\tabcolsep{2pt}
%\centering
%\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
%\begin{tabular}{@{}c|cccc@{}}
%\toprule
%            & LPIPS↓   &dists↓  &CLIPIQA↑   & MUSIQ↑  \\ \midrule
%SD3 w/ Controlnet&0.5618&0.2832&0.6092&	61.04 \\
%DACLIP-UIR&0.5986&0.3528 &0.3526&47.50 \\
%DPIR (ours) &\textbf{0.3903}&\textbf{0.1998}&\textbf{0.6424} &	\textbf{62.95}
%\\ \bottomrule
%\end{tabular}
%end{adjustbox}
%\vspace{-1em}
%\caption{Quantitative comparison in DrealSR dataset.}
%\vspace{-2em}
%\label{tab:control}
%\end{table}

\begin{table}[htbp]
\vspace{-4mm}
\setlength\tabcolsep{2pt}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\begin{tabular}{@{}c|cccc@{}}
\toprule
            & LPIPS↓ & DISTS↓ & CLIPIQA↑ & MUSIQ↑ \\ \midrule
ControlNet  & 0.5618 & 0.2832 & 0.6092   & 61.04  \\
DPIR (ours) & \textbf{0.3903} & \textbf{0.1998} & \textbf{0.6424} & \textbf{62.95} \\
\bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-3mm}
\caption{Comparison with SD3 ControlNet on DrealSR.}
\vspace{-4mm}
\label{tab:reb_controlnet}
\end{table}


==> tables/Kbjy_Q4.tex <==
\begin{table}[htbp]
\vspace{-4mm}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\begin{tabular}{@{}c|cccc@{}}
\toprule
      & PSNR↑ & SSIM↑  & LPIPS↓ & DISTS↓ \\ \midrule
SeeSR & 29.35 & 0.7695 & 0.2542 & 0.1542 \\
DPIR (ours) & \textbf{29.58}& \textbf{0.7739} & \textbf{0.2449}& \textbf{0.1302} \\
\bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-3mm}
\caption{Comparison with SeeSR on CelebA.}
\label{tab:reb_seesr}
\vspace{-4mm}
\end{table}


==> tables/e3SY_Q1.tex <==

\begin{table}[htbp]
%\vspace{-4mm}
\setlength\tabcolsep{2pt}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\begin{tabular}{@{}c|cccc@{}}
\toprule
                           & PSNR↑ & CLIPIQA↑ & MUSIQ↑ & MANIQA↑  \\ \midrule
DPIR w/o feature alignment & 27.00 & 0.478    & 47.87  & 0.2721   \\
%DPIR w/o any prompts       & \textbf{27.71} & 0.5199 & 55.78 & 0.2918 \\
DPIR w/ only light LQ cond & \textbf{27.71} & 0.5199 & 55.78 & 0.2918 \\
DPIR (ours)                & 27.31 & \textbf{0.6424} & \textbf{62.95} & \textbf{0.3880} \\ \bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-3mm}
%\caption{Ablation study about feature alignment and prompts.}
\caption{Ablation study about lightweight conditioning.}
\label{tab:reb_convnext}
%\vspace{-4mm}
\end{table}


==> tables/e3SY_Q2.tex <==

\begin{table}[htbp]
\vspace{-4mm}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}c|cccccccc@{}}
\toprule
                      & LPIPS↓ & CLIPIQA↑ & MUSIQ↑ & MANIQA↑  \\ \midrule
%Original VAE          & 0.4217 & 0.5614   & 57.08  & 0.3346   \\
L1 loss               & 0.5760 & 0.4341   & 51.00  & 0.3260   \\
L1 + LPIPS loss       & 0.4081 & 0.5327	  & 53.89  & 0.3275   \\
L1 + LPIPS + GAN loss & \textbf{0.3780} & \textbf{0.6306} & \textbf{60.76} & \textbf{0.3657}
\\ \bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-0.3cm}
\caption{Ablation study about DRE loss.}
\label{tab:reb_dre}
\vspace{-0.7cm}
\end{table}


==> tables/xuee_Q1.tex <==

\begin{table}[htbp]
\vspace{-4mm}
\setlength\tabcolsep{2pt}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\begin{tabular}{@{}c|cccc@{}}
\toprule
              & LPIPS↓ &DISTS↓  &CLIPIQA↑ & MUSIQ↑ \\ \midrule
DACLIP & 0.5712 & 0.3496 &0.3478   &45.36  \\
DACLIP-UIR & 0.5686 & 0.3528 &0.3526   &	47.50  \\
DPIR (ours)  &\textbf{0.3903}&\textbf{0.1998}&\textbf{0.6424} &	\textbf{62.95}
   \\ \bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-3mm}
\caption{Comparison with DACLIP on DrealSR.}
\vspace{-4mm}
\label{tab:reb_daclip}
\end{table}


==> tables/xuee_Q3.tex <==

\begin{table}[htbp]
\vspace{-4mm}
\centering
\footnotesize
%\begin{adjustbox}{width=.47\textwidth}
\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}c|cccccccc@{}}
\toprule
         & PSNR↑ & LPIPS↓ &CLIPIQA↑   & MUSIQ↑  \\ \midrule
DACLIP&32.84 &	0.1983	&0.4363
	&	46.33
 \\
 DPIR (ours)&	\textbf{35.46}&\textbf{0.1808}&\textbf{0.5150}&\textbf{57.96}

   \\ \bottomrule
\end{tabular}
%end{adjustbox}
\vspace{-3mm}
\caption{Comparison with DACLIP on PolyU.}
\label{tab:reb_denoising}
\vspace{-4mm}
\end{table}


==> vision_div2k.tex <==
\begin{figure*}[t]
    \centering
    % 第一行三张子图
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_lr.png}
    %     \label{fig:sub1}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_real.png}
    %     \label{fig:sub2}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_sta.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_sin.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_supir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/div2k/0805_dpir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    
    % 第二行三张子图
    \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_lr.png}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0807_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_lr.png}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0808_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_lr.png}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0820_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_lr.png}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0887_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_lr.png}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/div2k/0822_dpir.png}
      
    \end{subfigure}


        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_lr.png}
        \caption*{LQ}
    
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_real.png}
        \caption*{Real-ESRGAN~\cite{wang2021real}}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_sta.png}
        \caption*{StableSR~\cite{wang2024exploiting}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_sin.png}
        \caption*{SinSR~\cite{wang2024sinsr}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_supir.png}
        \caption*{SUPIR~\cite{yu2024scaling}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_dpir.png}
        \caption*{DPIR(Ours)}
      
    \end{subfigure}

    \caption{Qualitative comparisons of different IR methods on DIV2k-val
    dataset.}
    \label{fig:supp_compare3}

    % \vspace{-4mm}
\end{figure*}

==> vision_drealsr.tex <==
\begin{figure*}[t]
    \centering
    % 第一行三张子图
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_lr.png}
    %     \label{fig:sub1}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_real.png}
    %     \label{fig:sub2}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_sta.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_sin.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_supir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/drealsr/Canon_14_x1_dpir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    
    % 第二行三张子图
    \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_lr.png}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1137_x1_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_lr.png}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/DSC_1286_x1_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_lr.png}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_118_x1_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_lr.png}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_57_x1_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_lr.png}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/IMG_140_x1_dpir.png}
      
    \end{subfigure}


        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_lr.png}
        \caption*{LQ}
     
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_real.png}
        \caption*{Real-ESRGAN~\cite{wang2021real}}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_sta.png}
        \caption*{StableSR~\cite{wang2024exploiting}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_sin.png}
        \caption*{SinSR~\cite{wang2024sinsr}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_supir.png}
        \caption*{SUPIR~\cite{yu2024scaling}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/drealsr/panasonic_233_x1_dpir.png}
        \caption*{DPIR(Ours)}
      
    \end{subfigure}

    \caption{Qualitative comparisons of different IR methods on DrealSR
    dataset.}
    \label{fig:supp_compare1}

    % \vspace{-4mm}
\end{figure*}

==> vision_face.tex <==
\begin{figure*}[t]
    \centering
    % 第一行三张子图
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_lr.jpg}
    %     \label{fig:sub1}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_real.jpg}
    %     \label{fig:sub2}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_sta.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_sin.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_supir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/18_dpir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    
    % 第二行三张子图
    \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_lr.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_real.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/20_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_lr.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_real.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/22_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_lr.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_real.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/36_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_lr.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_real.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/40_dpir.png}
      
    \end{subfigure}

    %     \vspace{-0.3cm} % 行间距
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_lr.jpg}
    %     \label{fig:sub1}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_real.jpg}
    %     \label{fig:sub2}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_sta.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_sin.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_supir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/face/44_dpir.png}
    %     \label{fig:sub3}
    % \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_lr.jpg}
        \caption*{LQ}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_real.jpg}
        \caption*{Real-ESRGAN~\cite{wang2021real}}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_sta.png}
        \caption*{StableSR~\cite{wang2024exploiting}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_sin.png}
        \caption*{SinSR~\cite{wang2024sinsr}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_supir.png}
        \caption*{SUPIR~\cite{yu2024scaling}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/face/48_dpir.png}
        \caption*{DPIR(Ours)}
      
    \end{subfigure}

    \caption{Qualitative comparisons of different IR methods on CelebA
    dataset.}
    \label{fig:supp_compare4}

    % \vspace{-4mm}
\end{figure*}

==> vision_realsr.tex <==
\begin{figure*}[t]
    \centering
    % 第一行三张子图
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_lr.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_real.jpg}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_sta.jpg}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_sin.jpg}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_supir.jpg}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_002_LR4_dpir.jpg}
      
    \end{subfigure}
    
    % 第二行三张子图
    \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_lr.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_003_LR4_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_lr.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_006_LR4_supir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_LR4_lr.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_LR4_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_LR4_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_LR4_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_LR4_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Canon_010_dpir.png}
      
    \end{subfigure}

    %     \vspace{-0.3cm} % 行间距
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_lr.png}
    %     \label{fig:sub1}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_real.png}
    %     \label{fig:sub2}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_sta.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_sin.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_supir.png}
    %     \label{fig:sub3}
    % \end{subfigure}
    %     % \hfill
    % \begin{subfigure}[b]{0.16\hsize}
    %     \centering
    %     \includegraphics[width=\hsize]{supplement/realsr/Canon_015_LR4_dpir.png}
    %     \label{fig:sub3}
    % \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_lr.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_real.png}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_sta.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_sin.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_supir.png}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_001_LR4_dpir_dpir.png}
      
    \end{subfigure}

        \vspace{-0.3cm} % 行间距
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_lr.png}
        \caption*{LQ}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_real.png}
        \caption*{Real-ESRGAN~\cite{wang2021real}}
      
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_sta.png}
        \caption*{StableSR~\cite{wang2024exploiting}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_sin.png}
        \caption*{SinSR~\cite{wang2024sinsr}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_supir.png}
        \caption*{SUPIR~\cite{yu2024scaling}}
      
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.16\hsize}
        \centering
        \includegraphics[width=\hsize]{supplement/realsr/Nikon_008_LR4_dpir.png}
        \caption*{DPIR(Ours)}
      
    \end{subfigure}

    \caption{Qualitative comparisons of different IR methods on RealSR
    dataset.}
    \label{fig:supp_compare2}

    % \vspace{-4mm}
\end{figure*}
